Object Proxy Patterns for Accelerating Distributed Applications

Workflow and serverless frameworks have empowered new approaches to distributed application design by abstracting compute resources. However, their typically limited or one-size-fits-all support for advanced data flow patterns leaves optimization to the application programmer -- optimization that becomes more difficult as data become larger. The transparent object proxy, which provides wide-area references that can resolve to data regardless of location, has been demonstrated as an effective low-level building block in such situations. Here we propose three high-level proxy-based programming patterns -- distributed futures, streaming, and ownership -- that make the power of the proxy pattern usable for more complex and dynamic distributed program structures. We motivate these patterns via careful review of application requirements and describe implementations of each pattern. We evaluate our implementations through a suite of benchmarks and by applying them in three substantial scientific applications, in which we demonstrate substantial improvements in runtime, throughput, and memory usage.

==> listings/streaming-consumer.tex <==
\lstset{escapeinside={(*}{*)}}
\begin{lstlisting}[
    style=PythonStyle,
    label={lst:streaming-consumer},
    caption={Example stream consumer code using Kafka for metadata. The bulk data transfer mechanism is determined by the producer (a \texttt{FooConnector} in \autoref{lst:streaming-producer}) and encoded in the event metadata.},
    float,
    floatplacement=t,
]
from proxystore.proxy import Proxy
from proxystore.stream import StreamConsumer
from proxystore.stream import KafkaSubscriber

subscriber = KafkaSubscriber('topic', ...)  

with StreamConsumer(subscriber) as consumer:
    for item in consumer: 
        assert isinstance(item, Proxy)  
\end{lstlisting}

==> listings/streaming-producer.tex <==
\lstset{escapeinside={(*}{*)}}
\begin{lstlisting}[
    style=PythonStyle,
    label={lst:streaming-producer},
    caption={Example stream producer code using Kafka for metadata and an arbitrary \texttt{FooConnector} for bulk data transfer.},
    float,
    floatplacement=t,
]
from proxystore.connectors import FooConnector
from proxystore.store import Store
from proxystore.stream import StreamProducer
from proxystore.stream import KafkaPublisher

store = {'topic': Store(..., FooConnector(...))}
publisher = KafkaPublisher(...)

with StreamProducer(publisher, store) as producer:
    for item in ...:
        producer.send('topic', item) 
\end{lstlisting}
